Optimality Conditions for Bilevel Imaging Learning Problems with Total Variation Regularization

We address the problem of optimal scale-dependent parameter learning in total variation image denoising. Such problems are formulated as bilevel optimization instances with total variation denoising problems as lower-level constraints. For the bilevel problem, we are able to derive M-stationarity conditions, after characterizing the corresponding Mordukhovich generalized normal cone and verifying suitable constraint qualification conditions. We also derive B-stationarity conditions, after investigating the Lipschitz continuity and directional differentiability of the lower-level solution operator. A characterization of the Bouligand subdifferential of the solution mapping, by means of a properly defined linear system, is provided as well. Based on this characterization, we propose a two-phase non-smooth trust-region algorithm for the numerical solution of the bilevel problem and test it computationally for two particular experimental settings.

==> experiments/faces_10/faces_10_cost_plot.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
  ylabel = {$\|u-\bar{u}\|^2$},
  title = {Scalar Cost},
  xlabel = {$\alpha$},
  grid=both
]

\addplot+[
  mark = {none}
] coordinates {
  (2.220446049250313e-16, 121.9343152900488)
  (0.001000000000000222, 113.50533340498073)
  (0.002000000000000222, 105.73065876064462)
  (0.003000000000000222, 98.58569194506781)
  (0.004000000000000222, 92.04452094809066)
  (0.005000000000000222, 86.07884780996729)
  (0.006000000000000222, 80.66212778441627)
  (0.007000000000000222, 75.76453930807975)
  (0.008000000000000222, 71.35949508903269)
  (0.009000000000000223, 67.4198488419047)
  (0.010000000000000222, 63.91831003681047)
  (0.011000000000000221, 60.825331556677426)
  (0.012000000000000222, 58.11501566283591)
  (0.013000000000000223, 55.76131738140778)
  (0.014000000000000222, 53.739862171425855)
  (0.015000000000000221, 52.02348936058892)
  (0.016000000000000222, 50.58824962455636)
  (0.017000000000000223, 49.40973937686448)
  (0.018000000000000224, 48.468305998712765)
  (0.01900000000000022, 47.74122994898647)
  (0.020000000000000222, 47.20945888978605)
  (0.021000000000000223, 46.85499121745661)
  (0.02200000000000022, 46.660678642556455)
  (0.02300000000000022, 46.612393428458525)
  (0.024000000000000223, 46.693818488485576)
  (0.025000000000000223, 46.892181233282535)
  (0.026000000000000224, 47.19603003655342)
  (0.027000000000000222, 47.594163934280374)
  (0.028000000000000223, 48.075525738026904)
  (0.029000000000000224, 48.63230786905148)
  (0.03000000000000022, 49.2579979093113)
  (0.031000000000000222, 49.94641871592172)
  (0.03200000000000022, 50.69120950527609)
  (0.033000000000000224, 51.48587262707377)
  (0.034000000000000224, 52.327231702484674)
  (0.035000000000000225, 53.20961393940854)
  (0.036000000000000226, 54.12768887387591)
  (0.03700000000000022, 55.07883592090656)
  (0.03800000000000022, 56.05781023698016)
  (0.03900000000000022, 57.063417884029214)
  (0.04000000000000022, 58.09365349807977)
  (0.041000000000000224, 59.146938709469296)
  (0.042000000000000225, 60.221117821870386)
  (0.043000000000000226, 61.3156612870672)
  (0.04400000000000022, 62.4290895310531)
  (0.04500000000000022, 63.56028463153748)
  (0.04600000000000022, 64.70670219135614)
  (0.04700000000000022, 65.86575729689372)
  (0.04800000000000022, 67.03734999051294)
  (0.049000000000000224, 68.22167830916965)
  (0.050000000000000225, 69.41844582144672)
  (0.051000000000000226, 70.62541073970131)
  (0.05200000000000023, 71.8422953001607)
  (0.05300000000000022, 73.06928861097599)
  (0.05400000000000022, 74.30616185980323)
  (0.05500000000000022, 75.55142662890265)
  (0.05600000000000022, 76.80440163726347)
  (0.057000000000000224, 78.06444631623216)
  (0.058000000000000225, 79.33271224517053)
  (0.059000000000000226, 80.60965903044969)
  (0.06000000000000022, 81.89399611861305)
  (0.06100000000000022, 83.18624320262637)
  (0.06200000000000022, 84.4847390445705)
  (0.06300000000000022, 85.78869058667244)
  (0.06400000000000022, 87.09886999453445)
  (0.06500000000000022, 88.41437820666533)
  (0.06600000000000023, 89.73579273884)
  (0.06700000000000023, 91.0616923269865)
  (0.06800000000000023, 92.39132636773354)
  (0.06900000000000023, 93.72527349316539)
  (0.07000000000000023, 95.06241644769571)
  (0.07100000000000023, 96.40390825330084)
  (0.07200000000000023, 97.74928571109575)
  (0.07300000000000022, 99.10028315814125)
  (0.07400000000000022, 100.45527432121882)
  (0.07500000000000022, 101.81497190988226)
  (0.07600000000000022, 103.17735829101379)
  (0.07700000000000022, 104.5424868372399)
  (0.07800000000000022, 105.90893764629486)
  (0.07900000000000022, 107.27687020102508)
  (0.08000000000000022, 108.64829582862683)
  (0.08100000000000022, 110.02302815632589)
  (0.08200000000000023, 111.39988297063901)
  (0.08300000000000023, 112.77930866199364)
  (0.08400000000000023, 114.16031710535488)
  (0.08500000000000023, 115.54435035766478)
  (0.08600000000000023, 116.93229284232294)
  (0.08700000000000023, 118.32297583210287)
  (0.08800000000000022, 119.71545479114442)
  (0.08900000000000022, 121.10920678044666)
  (0.09000000000000022, 122.50410558935332)
  (0.09100000000000022, 123.90124643917258)
  (0.09200000000000022, 125.30056200963976)
  (0.09300000000000022, 126.70125039825334)
  (0.09400000000000022, 128.10320114566542)
  (0.09500000000000022, 129.50678536811716)
  (0.09600000000000022, 130.91081670050076)
  (0.09700000000000022, 132.31592890788247)
  (0.09800000000000023, 133.7219732457747)
  (0.09900000000000023, 135.12928630178098)
  (0.10000000000000023, 136.53716313501093)
  (0.10100000000000023, 137.94461634442376)
  (0.10200000000000023, 139.35124791158918)
  (0.10300000000000023, 140.75827603403582)
  (0.10400000000000023, 142.16370919102934)
  (0.10500000000000022, 143.56810572436578)
  (0.10600000000000022, 144.97218427374517)
  (0.10700000000000022, 146.37665102569267)
  (0.10800000000000022, 147.78019100868232)
  (0.10900000000000022, 149.18367388116533)
  (0.11000000000000022, 150.58819889749023)
  (0.11100000000000022, 151.9946671297546)
  (0.11200000000000022, 153.40195874356166)
  (0.11300000000000023, 154.8075377635549)
  (0.11400000000000023, 156.2131740005254)
  (0.11500000000000023, 157.61940589559023)
  (0.11600000000000023, 159.02561001979737)
  (0.11700000000000023, 160.43336979986242)
  (0.11800000000000023, 161.84012025106614)
  (0.11900000000000023, 163.24658570789344)
  (0.12000000000000022, 164.65281481163842)
  (0.12100000000000022, 166.058099342066)
  (0.12200000000000022, 167.46375582089368)
  (0.12300000000000022, 168.86982897061338)
  (0.12400000000000022, 170.27632155176337)
  (0.12500000000000022, 171.68334720342668)
  (0.12600000000000022, 173.09067040587314)
  (0.12700000000000022, 174.4985651166335)
  (0.12800000000000022, 175.90737193249066)
  (0.12900000000000023, 177.31594556339337)
  (0.13000000000000023, 178.72344751152772)
  (0.13100000000000023, 180.12889767785566)
  (0.13200000000000023, 181.53330756174967)
  (0.13300000000000023, 182.93835859227477)
  (0.13400000000000023, 184.34503231439317)
  (0.13500000000000023, 185.75159017862208)
  (0.13600000000000023, 187.1575477768119)
  (0.13700000000000023, 188.56383782964684)
  (0.13800000000000023, 189.97136844835086)
  (0.13900000000000023, 191.38092430405447)
  (0.14000000000000024, 192.7920825312008)
  (0.14100000000000024, 194.2040111280581)
  (0.14200000000000024, 195.6154896830222)
  (0.14300000000000024, 197.02658008075812)
  (0.14400000000000024, 198.43806152304435)
  (0.1450000000000002, 199.84973723604975)
  (0.1460000000000002, 201.26331734093472)
  (0.1470000000000002, 202.67812583310396)
  (0.14800000000000021, 204.09382324967478)
  (0.14900000000000022, 205.50878206599583)
  (0.15000000000000022, 206.9233816511783)
  (0.15100000000000022, 208.33800191283447)
  (0.15200000000000022, 209.75419864174532)
  (0.15300000000000022, 211.17012042683803)
  (0.15400000000000022, 212.58635374160647)
  (0.15500000000000022, 214.00306020390966)
  (0.15600000000000022, 215.4195754063677)
  (0.15700000000000022, 216.83670812195027)
  (0.15800000000000022, 218.25415812789885)
  (0.15900000000000022, 219.67092427916683)
  (0.16000000000000023, 221.08790171368616)
  (0.16100000000000023, 222.50472620213557)
  (0.16200000000000023, 223.92141209233841)
  (0.16300000000000023, 225.33826525158221)
  (0.16400000000000023, 226.75512889864908)
  (0.16500000000000023, 228.17155955130872)
  (0.16600000000000023, 229.58790761391273)
  (0.16700000000000023, 231.0008101990316)
  (0.16800000000000023, 232.41284323511636)
  (0.16900000000000023, 233.8243293500461)
  (0.17000000000000023, 235.23450840696353)
  (0.17100000000000024, 236.64408356124545)
  (0.17200000000000024, 238.05240362979285)
  (0.17300000000000024, 239.46012528937342)
  (0.17400000000000024, 240.86585535943337)
  (0.17500000000000024, 242.27024225812585)
  (0.1760000000000002, 243.67377186437162)
  (0.1770000000000002, 245.0768552925335)
  (0.1780000000000002, 246.47971816292804)
  (0.17900000000000021, 247.88188278663523)
  (0.18000000000000022, 249.28199933827753)
  (0.18100000000000022, 250.68059464956144)
  (0.18200000000000022, 252.07797155799318)
  (0.18300000000000022, 253.47522413564758)
  (0.18400000000000022, 254.87199308814144)
  (0.18500000000000022, 256.2668250899744)
  (0.18600000000000022, 257.6604818843693)
  (0.18700000000000022, 259.0540048645188)
  (0.18800000000000022, 260.4479807871399)
  (0.18900000000000022, 261.8420951591517)
  (0.19000000000000022, 263.2345718776396)
  (0.19100000000000023, 264.6253743229992)
  (0.19200000000000023, 266.015142681767)
  (0.19300000000000023, 267.404790621829)
  (0.19400000000000023, 268.7933372937429)
  (0.19500000000000023, 270.1826850300043)
  (0.19600000000000023, 271.57184900639623)
  (0.19700000000000023, 272.9609518503978)
  (0.19800000000000023, 274.34539255918185)
  (0.19900000000000023, 275.7278944812658)
};

\addplot+[
] coordinates {
  (0.022849548339843973, 46.63300207498421)
};

\end{axis}
\end{tikzpicture}



==> experiments/faces_10/faces_10_cost_plot_2d.tex <==
\begin{tikzpicture}[scale=0.8]
\begin{axis}[
  ylabel = {$\alpha_2$},
  title = {2D Cost},
  xlabel = {$\alpha_1$},
  grid=both,
  view = {{0}{90}}
]

\addplot3[
  contour prepared,
  dashed
] table {
  0.024 0.024056383719925103 46.7
  0.023 0.024345387065936495 46.7
  0.022 0.02405744567348299 46.7
  0.02193880120893651 0.024 46.7
  0.02145519397592663 0.023 46.7
  0.021617831821712067 0.022 46.7
  0.022 0.02156951546549227 46.7
  0.023 0.02122269383549772 46.7
  0.024 0.021569068930197253 46.7
  0.02444330157359196 0.022 46.7
  0.024630671309295096 0.023 46.7
  0.02406962745172512 0.024 46.7
  0.024 0.024056383719925103 46.7

  0.028062186610990095 0.024 47.35
  0.02825271088430656 0.023 47.35
  0.028189641921571463 0.022 47.35
  0.028 0.021455011199527897 47.35
  0.027816575897086724 0.021 47.35
  0.027055486972958665 0.02 47.35
  0.027 0.019951999666486222 47.35
  0.026 0.019243019648512927 47.35
  0.02554525710138293 0.019 47.35
  0.025 0.018788192005385913 47.35
  0.024 0.018542295191910294 47.35
  0.023 0.01845508421862125 47.35
  0.022 0.018543834180713082 47.35
  0.021 0.018830350235893516 47.35
  0.020665094415919773 0.019 47.35
  0.02 0.01946316242053452 47.35
  0.019479142450242223 0.02 47.35
  0.019 0.02074950064502857 47.35
  0.018882115268835355 0.021 47.35
  0.018631899959386685 0.022 47.35
  0.01858544305515429 0.023 47.35
  0.018720748430403354 0.024 47.35
  0.019 0.024933788562892585 47.35
  0.019026903867617875 0.025 47.35
  0.01963548881705208 0.026 47.35
  0.02 0.026461328441652686 47.35
  0.02063041296927467 0.027 47.35
  0.021 0.027262402484796115 47.35
  0.022 0.027663398847718644 47.35
  0.023 0.027786544304026342 47.35
  0.024 0.027663306653233678 47.35
  0.025 0.027317131872696354 47.35
  0.025580201976512975 0.027 47.35
  0.026 0.026723713685019666 47.35
  0.026830406771360022 0.026 47.35
  0.027 0.02580813334788465 47.35
  0.027586792825536378 0.025 47.35
  0.028 0.02414853918259129 47.35
  0.028062186610990095 0.024 47.35

  0.03 0.020699005124514547 48.0
  0.029592868436964837 0.02 48.0
  0.029 0.019329529605260354 48.0
  0.02867151297641078 0.019 48.0
  0.028 0.018510187868308964 48.0
  0.027188088190466034 0.018 48.0
  0.027 0.0179090098272861 48.0
  0.026 0.01751254950092175 48.0
  0.025 0.017213645879953672 48.0
  0.024 0.017024702669993275 48.0
  0.023630520381088753 0.017 48.0
  0.023 0.016966409402040847 48.0
  0.022387179523393214 0.017 48.0
  0.022 0.017026620645847583 48.0
  0.021 0.017247872414456012 48.0
  0.02 0.017638560446255676 48.0
  0.019375056289962913 0.018 48.0
  0.019 0.01828132650472147 48.0
  0.018294531442212394 0.019 48.0
  0.018 0.019412184868647188 48.0
  0.017674624135775783 0.02 48.0
  0.017309719131837535 0.021 48.0
  0.01711577872261788 0.022 48.0
  0.017079734903875633 0.023 48.0
  0.01718441808447498 0.024 48.0
  0.017416064808199634 0.025 48.0
  0.017762927958909897 0.026 48.0
  0.018 0.02652640053063709 48.0
  0.018275452948790127 0.027 48.0
  0.01897525238481137 0.028 48.0
  0.019 0.028030666050375706 48.0
  0.02 0.028942616920319544 48.0
  0.020093188298428596 0.029 48.0
  0.021 0.029498665895359426 48.0
  0.022 0.029809564375692127 48.0
  0.023 0.029905324308856954 48.0
  0.024 0.029810413123197103 48.0
  0.025 0.02954302367358815 48.0
  0.026 0.02912035673048877 48.0
  0.02621498181401723 0.029 48.0
  0.027 0.028507351290723567 48.0
  0.027664767566140287 0.028 48.0
  0.028 0.027704908750172244 48.0
  0.02868969900519762 0.027 48.0
  0.029 0.026618098136615396 48.0
  0.029445128485567216 0.026 48.0
  0.029999589493837634 0.025 48.0
  0.03 0.02499889380509949 48.0

  0.03 0.018250095099177372 48.65
  0.029695907102884864 0.018 48.65
  0.029 0.017559194993545944 48.65
  0.028004045192089242 0.017 48.65
  0.028 0.01699819074474202 48.65
  0.027 0.01661297826622081 48.65
  0.026 0.016297326255775353 48.65
  0.025 0.016059422999514003 48.65
  0.024604621791688323 0.016 48.65
  0.024 0.015925472705674217 48.65
  0.023 0.01588205327879334 48.65
  0.022 0.01592728683156633 48.65
  0.02149814206061634 0.016 48.65
  0.021 0.016087958776669947 48.65
  0.02 0.016399659452909134 48.65
  0.019 0.016860890336957143 48.65
  0.018777928399562927 0.017 48.65
  0.018 0.01761121665817158 48.65
  0.01761657554970147 0.018 48.65
  0.017 0.018810604265451975 48.65
  0.01688454409845723 0.019 48.65
  0.01644070256238913 0.02 48.65
  0.01614811884002711 0.021 48.65
  0.016 0.02195333780902866 48.65
  0.015994038472415918 0.022 48.65
  0.01597028461129611 0.023 48.65
  0.016 0.02343108950546214 48.65
  0.01604768941853612 0.024 48.65
  0.016233285400359322 0.025 48.65
  0.01651125779423388 0.026 48.65
  0.016872141228234272 0.027 48.65
  0.017 0.02729438068190832 48.65
  0.017382537114504288 0.028 48.65
  0.018 0.028987641987356774 48.65
  0.01800997381959841 0.029 48.65
  0.018913917265198452 0.03 48.65

  0.027771214145545123 0.03 48.65
  0.028 0.02984410267010721 48.65
  0.029 0.029053486324737234 48.65
  0.029059986463817234 0.029 48.65
  0.03 0.02806071060968196 48.65

  0.017336042905617736 0.03 49.3
  0.017 0.029520285627348077 49.3
  0.01670796110313475 0.029 49.3
  0.016206955108608055 0.028 49.3
  0.016 0.027523663819610984 49.3
  0.015812883607817862 0.027 49.3
  0.015516035294866315 0.026 49.3
  0.015287427431387009 0.025 49.3
  0.015134765120497221 0.024 49.3
  0.015065727328738293 0.023 49.3
  0.01508959275501938 0.022 49.3
  0.015217471087196208 0.021 49.3
  0.015458133114045139 0.02 49.3
  0.015823377054743407 0.019 49.3
  0.016 0.018647874644699976 49.3
  0.01639502579591925 0.018 49.3
  0.017 0.017234705676656775 49.3
  0.017231472065501185 0.017 49.3
  0.018 0.016378647925837528 49.3
  0.01860433113140497 0.016 49.3
  0.019 0.015796556532738485 49.3
  0.02 0.015417914277681643 49.3
  0.021 0.015161965173762858 49.3
  0.022 0.015016803463728978 49.3
  0.02236958944538648 0.015 49.3
  0.023 0.014976053919363118 49.3
  0.023665608703161603 0.015 49.3
  0.024 0.01501440839870511 49.3
  0.025 0.015137431200285576 49.3
  0.026 0.015332307620399785 49.3
  0.027 0.015590998494469223 49.3
  0.028 0.015906800849618045 49.3
  0.0282541324672279 0.016 49.3
  0.029 0.01633351634056722 49.3
  0.03 0.01683795461431744 49.3

  0.03 0.015775116827713122 49.95
  0.029 0.01536140963778711 49.95
  0.028014269036100957 0.015 49.95
  0.028 0.014995632233266129 49.95
  0.027 0.0147320614425214 49.95
  0.026 0.014516300863252191 49.95
  0.025 0.014353734211333988 49.95
  0.024 0.014251187383731519 49.95
  0.023 0.014215370886934819 49.95
  0.022 0.014253612318339902 49.95
  0.021 0.014375114746784112 49.95
  0.02 0.014589076420203911 49.95
  0.019 0.014905547499666324 49.95
  0.01878016140317452 0.015 49.95
  0.018 0.015401255976950017 49.95
  0.017097719503555042 0.016 49.95
  0.017 0.016079012931868687 49.95
  0.01608689775772563 0.017 49.95
  0.016 0.01710991565937995 49.95
  0.015421138417093186 0.018 49.95
  0.015 0.018839270679373073 49.95
  0.014932429764302469 0.019 49.95
  0.014626444622341495 0.02 49.95
  0.014424786715465007 0.021 49.95
  0.014317618905639947 0.022 49.95
  0.014297674337096607 0.023 49.95
  0.014355506117982367 0.024 49.95
  0.014483395355071284 0.025 49.95
  0.014674881847571066 0.026 49.95
  0.01492353581535988 0.027 49.95
  0.015 0.027255450507971672 49.95
  0.015266131430931817 0.028 49.95
  0.015678300206137825 0.029 49.95
  0.016 0.029696703234312526 49.95
  0.016170271928766532 0.03 49.95

  0.03 0.014885528423320851 50.6
  0.029 0.014540094426797209 50.6
  0.028 0.014234084092033122 50.6
  0.02711148737913009 0.014 50.6
  0.027 0.013975085013951088 50.6
  0.026 0.01379223235679648 50.6
  0.025 0.013654461818766901 50.6
  0.024 0.01356759167821361 50.6
  0.023 0.013537357379330945 50.6
  0.022 0.013569993324124348 50.6
  0.021 0.013673281858792933 50.6
  0.02 0.013855016332597283 50.6
  0.01946066426219911 0.014 50.6
  0.019 0.014145888422562468 50.6
  0.018 0.014575664489047393 50.6
  0.017234627049163946 0.015 50.6
  0.017 0.015155720032669923 50.6
  0.016 0.015983571585154583 50.6
  0.015983673897083592 0.016 50.6
  0.01516800376926624 0.017 50.6
  0.015 0.017258293627943042 50.6
  0.01459578277563098 0.018 50.6
  0.01417531531834242 0.019 50.6
  0.014 0.019572782929195343 50.6
  0.013888861112666748 0.02 50.6
  0.013717405364641685 0.021 50.6
  0.013626306974284587 0.022 50.6
  0.013609377774443087 0.023 50.6
  0.013658536432313526 0.024 50.6
  0.013767248586560867 0.025 50.6
  0.013930041770317265 0.026 50.6
  0.014 0.026330852238632352 50.6
  0.014166463161930721 0.027 50.6
  0.014465838907685045 0.028 50.6
  0.014811105776976417 0.029 50.6
  0.015 0.029488319714101405 50.6
  0.01523630902563586 0.03 50.6

  0.03 0.014123747021326512 51.25
  0.02964170255498947 0.014 51.25
  0.029 0.013811984113635168 51.25
  0.028 0.013552506291116507 51.25
  0.027 0.013329097676601396 51.25
  0.026 0.013146377842486111 51.25
  0.025 0.013008828058652064 51.25
  0.024898262174294677 0.013 51.25
  0.024 0.012933037796757078 51.25
  0.023 0.012907192698885423 51.25
  0.022 0.012935384948021331 51.25
  0.021273258485858218 0.013 51.25
  0.021 0.013028265456799812 51.25
  0.02 0.013210190678980977 51.25
  0.019 0.013479182146454004 51.25
  0.018 0.013844070013585695 51.25
  0.01766868886633021 0.014 51.25
  0.017 0.014370799835277535 51.25
  0.01609034180472096 0.015 51.25
  0.016 0.015074794695346562 51.25
  0.015080556635274377 0.016 51.25
  0.015 0.016098753566620095 51.25
  0.01438403472129598 0.017 51.25
  0.014 0.017704431679409913 51.25
  0.013862993086521612 0.018 51.25
  0.013505553736413982 0.019 51.25
  0.013245360179929477 0.02 51.25
  0.013073840057570233 0.021 51.25
  0.013 0.02181045604470553 51.25
  0.012985175637596229 0.022 51.25
  0.012970644191354824 0.023 51.25
  0.013 0.02369543054091107 51.25
  0.01301497676772521 0.024 51.25
  0.013123703396786323 0.025 51.25
  0.01328654528052254 0.026 51.25
  0.01349807359933103 0.027 51.25
  0.013752549217325466 0.028 51.25
  0.014 0.028843151725608394 51.25
  0.014054160663946545 0.029 51.25
  0.014441012629404724 0.03 51.25

  0.03 0.013458678831692057 51.9
  0.029 0.013165734790975745 51.9
  0.028360935167450932 0.013 51.9
  0.028 0.012919586251724615 51.9
  0.027 0.012727726456915655 51.9
  0.026 0.012570855969837858 51.9
  0.025 0.012452809260301307 51.9
  0.024 0.012378373647390657 51.9
  0.023 0.012352644655869074 51.9
  0.022 0.01238096080222322 51.9
  0.021 0.012469995881314328 51.9
  0.02 0.012626473305922222 51.9
  0.019 0.012857821492861377 51.9
  0.018546952434863467 0.013 51.9
  0.018 0.013199657448021665 51.9
  0.017 0.013670392325879584 51.9
  0.016438618546711914 0.014 51.9
  0.016 0.014303423755101663 51.9
  0.01517151474585551 0.015 51.9
  0.015 0.015172589193721081 51.9
  0.014311008126686798 0.016 51.9
  0.014 0.016454992713122965 51.9
  0.013683213463954298 0.017 51.9
  0.01321962239380519 0.018 51.9
  0.013 0.01861433999838792 51.9
  0.012881628832878248 0.019 51.9
  0.01265820764815112 0.02 51.9
  0.012510937033758543 0.021 51.9
  0.012432721605114315 0.022 51.9
  0.012418188613310541 0.023 51.9
  0.012460406141414774 0.024 51.9
  0.01255376263919291 0.025 51.9
  0.012693583642893936 0.026 51.9
  0.012875246139706567 0.027 51.9
  0.013 0.027570927352524054 51.9
  0.0131092052195552 0.028 51.9
  0.013402727688758753 0.029 51.9
  0.01373158529912847 0.03 51.9

};

\addplot+[
] coordinates {
  (0.02298057745857323, 0.02273441356170018)
};

\end{axis}
\end{tikzpicture}


